Constraining the top electroweak sector of the SMEFT through $Z$ associated top pair and single top production at the HL-LHC

We study the processes $pp \to t\bar{t}Z$ and $pp \to tZj$ in the framework of Standard Model Effective Field Theory (SMEFT), employing conventional cut-and-count as well as machine learning techniques to take advantage of kinematic information in complex final states involving multiple leptons and $b$ jets. We explore the projected sensitivity for two SMEFT operators, $\mathcal{O}_{tZ}$ and $\mathcal{O}_{tW}$, that induce electroweak dipole moment interactions for top quarks, through direct searches in these electroweak top production processes at the HL-LHC. New physics modifications to dominant backgrounds are also considered. We show that the new physics sensitivity can be enhanced through a combination of differential distributions for relevant kinematic observables and machine learning techniques. Searches in $t\bar{t}Z$ and $tZj$ production result in stronger constraints on $\mathcal{C}_{tZ}$ and $\mathcal{C}_{tW}$, respectively. At the HL-LHC, $\mathcal{C}_{tZ}$ can be probed up to $-0.41 \lesssim \mathcal{C}_{tZ} \lesssim 0.47$ through searches in the $pp \to t\bar{t}Z + tWZ \to 3\ell + 2b\ + \geq 2j$ channel while $\mathcal{C}_{tW}$ can be probed up to $-0.14 \lesssim \mathcal{C}_{tW} < 0.11$ from searches in the $pp \to tZj + t\bar{t}Z + tWZ \to 3\ell + 1b + 1/2j$ channel, at $95\%$ CL.

==> header.tex <==
\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx,tabularx}
\usepackage{color}
\usepackage{multirow}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{slashed}
\usepackage[normalem]{ulem}
\usepackage{scalerel}
\usepackage{soul}

\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

\newcommand{\be}{\begin{equation} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\def\figureautorefname~#1\null{Fig.\,#1\null}
\def\tableautorefname~#1\null{Tab.\,#1\null}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\def\equationautorefname~#1\null{Eq.\,(#1)\null}

% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}
\newcommand{\br}{\mathrm{BR}}

% Units
\newcommand{\ev}{\text{eV}}
\newcommand{\kev}{\text{keV}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}

\newcommand{\ab}{\text{ab}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\pb}{\text{pb}}
\newcommand{\ipb}{\text{pb}^{-1}}

\newcommand{\nm}{\text{nm}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}

\newcommand{\mrad}{\text{mrad}}
\newcommand{\murad}{\mu\text{rad}}

\newcommand{\g}{\text{g}}
\newcommand{\kg}{\text{kg}}
\newcommand{\ton}{\text{t}}
\newcommand{\sr}{\text{sr}}
\newcommand{\ns}{\text{ns}}

\newcommand{\fasernu}{FASER$\nu$~}

\newcommand{\Eqref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\Eqsref}[2]{Equations~(\ref{eq:#1}) and (\ref{eq:#2})}
\renewcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\eqsref}[2]{Eqs.~(\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\secsref}[2]{Secs.~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Secsref}[2]{Sections~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figsref}[2]{Figs.~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\figssref}[3]{Figs.~\ref{fig:#1}, \ref{fig:#2} and \ref{fig:#3}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tableref}[1]{Table~\ref{table:#1}}
\newcommand{\tablesref}[2]{Tables~\ref{table:#1} and \ref{table:#2}}
\newcommand{\appref}[1]{Appendix~\ref{sec:#1}}
\newcommand{\appsref}[2]{Appendices~\ref{sec:#1} and \ref{sec:#2}}


%comments
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}

\newcommand{\rb}[1]{\textcolor{blue}{{#1}}}
\newcommand{\AI}[1]{\textcolor{red}{{#1}}}

\crefname{section}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{appendix}{Appendix}{Appendices}
\crefname{table}{Table}{Tables}

%Ref Style
\bibliographystyle{utphys}

